Lognormals, Power Laws and Double Power Laws in the Distribution of Frequencies of Harmonic Codewords from Classical Music

Zipf's law is a paradigm describing the importance of different elements in communication systems, especially in linguistics. Despite the complexity of the hierarchical structure of language, music has in some sense an even more complex structure, due to its multidimensional character (melody, harmony, rhythm, timbre...). Thus, the relevance of Zipf's law in music is still an open question. Using discrete codewords representing harmonic content obtained from a large-scale analysis of classical composers, we show that a nearly universal Zipf-like law holds at a qualitative level. However, in an in-depth quantitative analysis, where we introduce the double power-law distribution as a new player in the classical debate between the superiority of Zipf's (power) law and that of the lognormal distribution, we conclude not only that universality does not hold, but that there is not a unique probability distribution that best describes the usage of the different codewords by each composer.

==> p_supplementary_info.tex <==
\title{
Supplementary Information:\\
Lognormals, Power Laws and Double Power Laws
in the Distribution of Frequencies
of Harmonic Codewords from 
Classical Music
%Lognormal, Power Law and Double Power Law
%Distributions of Frequencies
%of Harmonic Codewords in 
%Classical Music
} 
\author{Marc Serra-Peralta}
\affiliation{%
Centre de Recerca Matem\`atica,
Edifici C, Campus Bellaterra,
E-08193 Barcelona, Spain
}
\affiliation{Departament de Física,
Facultat de Ci\`encies,
Universitat Aut\`onoma de Barcelona,
E-08193 Barcelona, Spain
}
\author{Joan Serr\`a}
\affiliation{Dolby Laboratories, E-08018 Barcelona, Spain}
\author{\'Alvaro Corral}
\affiliation{%
Centre de Recerca Matem\`atica,
Edifici C, Campus Bellaterra,
E-08193 Barcelona, Spain
}\affiliation{Departament de Matem\`atiques,
Facultat de Ci\`encies,
Universitat Aut\`onoma de Barcelona,
E-08193 Barcelona, Spain}
%\affiliation{Barcelona Graduate School of Mathematics, 
%Edifici C, Campus Bellaterra,
%E-08193 Barcelona, Spain}
\affiliation{Complexity Science Hub Vienna,
Josefst\"adter Stra$\beta$e 39,
1080 Vienna,
Austria
}

\maketitle


\section{Data Processing and Fitting}


\subsection{Data Cleaning and Detection of Repeated Pieces}

As mentioned before, very short pieces are removed, and for us this is given by a number of beats below or equal to 15.
In order to identify files corresponding to repeated pieces, we check if two or more files 
yield the same values of $L$ and $V$. 
As this is not enough to characterize a repetition, we do the same analysis
for bigrams, trigrams, and quadrigrams
(a bigram is a concatenation of two codewords, a trigram of three, etc.),
and the pieces having the same values of $L$ and $V$ from unigrams (our standard codewords)
to quadrigrams are visually inspected, and the repeated ones removed.
The number of repetitions was found to be 212.
The resulting final values of $L$ and $V$ for the global corpus
(76 composers with 9327 pieces) are $L=5,088,442$
%$L=5,131,151$ 
%(A MI EM SURT 5,078,287) ????
and $V=4085$.


%one can 
%count the number of different codewords (or
% types), denoted as $V$
%(from ``vocabulary'')
%and also
%count its length
%in units of time intervals (number of tokens of music codewords), denoting it as $L$.

%MOSTRAR LA TIME SERIES DE UNA PIEZA??? EN BINARIO?? POR RANGOS??


\subsection{Harmonic Codewords}

The elementary entities %that are considered the building blocks of music
%that will constitute the building blocks of each musical piece
of which each musical piece is composed 
are defined as in Ref.~\cite{Serra_Corral_richness} 
(in a similar way as it was done before in Ref. \cite{Serra_scirep}).
A summary of the procedure to obtain them follows:
%The idea of the procedure 
%is explained in detail in Ref. \cite{Serra_Corral_richness}, but the idea 
%is as follows:

\begin{enumerate}[(i)]
\item Starting with a MIDI file, corresponding to the score of a piece,
this is converted
by means of the {\tt midi2abc} program \cite{midi2abc}
into a standard readable text file,
containing the time occurrence, duration, and pitch of each note.
\item All pitches are transformed into pitch classes, 
which removes the distinction between different octaves.
This leads to 12 pitch classes, $C$, $C\#$, etc., up to $A\#$ and $B$.
\item The piece is divided into time intervals
corresponding to beats, as the beat is the fundamental time scale in music.
%{and the length of them is given by one beat
%using the beats to define the time intervals
%(as this is the fundamental time scale in music).}
Silent time intervals
at the beginning and at the end of the piece are removed.
\item %For each of these time intervals  
%%each beat, 
%we construct a 12-dimensional vector (called chroma)
%with one component for each pitch class, 
%$(C,C\#,\dots G\#, A,A\#,B)$.
For each time interval,
the sum of the duration of all the notes 
of a given pitch class
%present in the time interval 
are assigned to one of the
12 components of a 12-dimensional vector (called chroma),
with each component associated to a pitch class, 
$(C,C\#,\dots G\#, A,A\#,B)$.
Notes that occupy more than one time interval
are split {proportionally between the intervals}.
The duration is measured in units of the time interval
(i.e., in units of beats).
\item The vectors are discretized,
with components below a fixed threshold (0.1 by default) reset to zero
and components above the threshold reassigned to one.
These ``discretized chromas'' yield the harmonic codewords
or types
that constitute 
the harmonic building blocks of the musical pieces. %, in our framework
%HACE FALTA EL THRESHOLD? qUE PASA SI ES 0???
Note that there are $2^{12}=4096$ possible types.
So, at this coarse-grained level,
each piece is represented as a 12-dimensional time series of binary elements.
\item {Each piece 
%(i.e.,  the chroma constituting the piece) 
is transposed;} 
major pieces to $C$ major and minor pieces to $A$ minor.
This constitutes a shift of the pitches by a constant amount 
(or a rescaling of the wavelengths, in physical terms), 
in order that the tonic note becomes pitch class $C$ 
(for major keys) or $A$ (minor keys).
Thus, pitch classes turn to represent in fact tonal functions.
See Ref. \cite{Serra_Corral_richness},
{which also details the method used for the determination of the key.}
\item All pieces corresponding to the same composer are aggregated.
This is done at the level of the time series of (transposed) discretized chromas.
The reason for aggregation 
is that many pieces are too short to provide a meaningful statistical analysis.
The resulting aggregation yields 76 datasets, one for each composer.
{An additional dataset, further aggregating the 76 individual datasets, is considered as representative of ``classical music'' as a whole.
We refer to it as the global dataset.}
%UN NOMBRE MEJOR????
%AGGREGATED NO ERA UN BUEN NOMBRE PORQUE LOS DE LOS COMPOSITORES INDIVIDUALES TAMBIEN SON AGGREGATED!!!
\end{enumerate}



Notice that step vi (transposition) would be irrelevant if we calculated the distribution of codeword counts for individual pieces, but it becomes very important as we aggregate the pieces, 
because they usually come in different keys
(transposition makes the key to be the same, for pieces in major and minor keys, separately). 



\subsection{Fitting Method}

For each dataset,
the absolute frequencies $n$ of each of the $V$ types 
provides the values of the random variable for which the statistical analysis is performed
%and the statistical  treatment is perfomed with $n$ as the random variable
(other approaches use the so-called rank as the random variable \cite{Altmann_Gerlach},
but there are good arguments in favor of using $n$ \cite{Corral_Cancho}).
The set of values of $n$ allow one to apply maximum-likelihood estimation
(once a fitting distribution is provided), 
as well as the Kolmogorov-Smirnov goodness-of-fit test
(the latter through the construction of the estimated cumulative distribution function).
%
In principle, 
a fit is accepted (in the sense that it is not rejected)
if the resulting $p-$value of the Kolmogorov-Smirnov test is greater than 0.20
(note that this is much stricter than the usual 0.05 significance level).
$p-$values are calculated from 100 Monte-Carlo simulations of the distribution resulting from the fit.

Fits are not performed for all $n\ge 1$, 
but above the lower cut-off $a$, greater than one in practice.
The reason is that it is nearly impossible that a simple probability distribution (with few parameters) fits well the smallest frequencies, for which the statistics is very high
(which is a common characteristics of Zipfian systems \cite{Corral_Cancho});
we systematically obtain $p=0$ if $a=1$.
Thus, fits are repeated for different values of the lower cut-off,
which are swept uniformly in log-scale 
(with 20 values per order of magnitude).
In the case of the truncated power-law, there is also an upper cut-off $b$ 
in the definition of the distribution, and, in the same way, 
different values of the upper cut-off are analyzed.

Among all non-rejectable fits 
(all with $p>0.20$, for different values of the cut-offs), 
the procedure we use selects
%the one %with the range 
%with the maximum number of counts 
%i.e., 
the one that includes more types.
If the resulting value of the lower cut-off $a$ is larger than 32, 
the fit is rejected (despite $p>0.20$),
due to the fact that more than one and a half orders of magnitude in frequencies (from $n=1$ to $10^{3/2}\simeq 32$) 
%$\sqrt{1000}\simeq 32$) 
would be excluded from the fit.
Thus, $p>0.20$ and $a\le 32$ is what we consider a ``good fit''.
%
{Note that
when we quantify the span of
the fitting range of a distribution 
we refer to the logarithmic span of the fitting range, 
$n_{max}/a$, 
with $n_{max}$ the maximum value of $n$ observed in the data.}
%
%LO DE VARIAR EL RANGO EXPLICARLO MEJOR ANTES!!!
%
An important thing about the fitting method
is that it is fully automatic and does not involve subjective judgements 
(so as to decide when the power-law regimes start).
More details 
%how the theoretical distributions are fitted to the empirical data 
are given in Refs. \cite{Corral_Deluca,Corral_Gonzalez}. 


\subsection{Model Selection}

%ACLARAR QUE ES UN BUEN FIT Y QUE ES EL MEJOR FIT, 
%FITTING RANGE ES LOGARITMICO!!

%(\textbf{POSAR AQUESTA SECCIÓ DESPRÉS DE "FITTING METHOD"??}) 
 
%both the double power-law and the lognormal 
When
more than one distribution 
fits the data, 
we need to decide which is the best fit, in order to select it 
as the one best explaining the data.
{For model comparison, it is important to correct 
for the different number of free parameters that each distribution may have
(the more parameters, the better the fit, in principle, but the improvement has to be significant).
For that purpose, it is common to use the Akaike and the Bayesian information criteria, or a likelihood-ratio test \cite{Clauset}.

The problem we deal with, however, has an extra ingredient that makes the situation more complicated:
each distribution fits a different subset of the data, in general,
given by different values of the lower cut-off $a$
for each distribution
{($a_\text{pl}$, $a_\text{dpl}$ and $a_\text{ln}$)}; 
i.e., only values of the random variable fulfilling $n\ge a$ are fitted
(the criteria mentioned in the previous paragraph 
compare fits acting over fixed data).}
%As, in general, each fit will yield a different value of the lower cut-off $a$
%and therefore the number of data fitted by each distribution will be different,
To overcome this difficulty,
we use the simple criterion of choosing the distribution that fits a larger number of data points
(i.e., more types), 
which is equivalent to select the one with the smaller lower cut-off $a$,
independently of the number of parameters.
This is what defines for us the ``best fit,''
and 
in this way, we give absolute priority to fitting the largest fraction of the dataset.

{The reason for our choice can be justified as follows.
If a distribution fits the data for $n\ge a$, then, the remainder $a-1$ empirical points (outside the fit) can be considered to be fitted using the $a-1$ values
of the empirical probabilities $f(n)$, from $f(1)$ to $f(a-1)$.
Thus, if the difference in $a-$values between two distributions is relatively large, 
as it is the usual case, the difference in the number of ``total parameters''
(including the empirical probabilities below $a$) is large as well
and the distribution with smaller $a$ has a much smaller number of ``total parameters.''
Note that, in any case, 
we are comparing distributions that already provide good fits 
($p>0.20$).
Moreover, we find more natural to prefer a distribution given by a simple formula,
than one containing empirical values of probabilities as free parameters.
}
%
In the case of two distributions yielding the same minimum value of the lower cut-off (tie), 
the distribution with a smaller number of parameters is selected as the best fit
{(we only find this situation in 7 cases).}



\bibliography{biblio} 
\bibliographystyle{unsrt}


